DIVA-DAF: A Deep Learning Framework for Historical Document Image Analysis

Deep learning methods have shown strong performance in solving tasks for historical document image analysis. However, despite current libraries and frameworks, programming an experiment or a set of experiments and executing them can be time-consuming. This is why we propose an open-source deep learning framework, DIVA-DAF, which is based on PyTorch Lightning and specifically designed for historical document analysis. Pre-implemented tasks such as segmentation and classification can be easily used or customized. It is also easy to create one's own tasks with the benefit of powerful modules for loading data, even large data sets, and different forms of ground truth. The applications conducted have demonstrated time savings for the programming of a document analysis task, as well as for different scenarios such as pre-training or changing the architecture. Thanks to its data module, the framework also allows to reduce the time of model training significantly.

==> sections/0X_features.tex <==
\section{Features}\label{sec:features}
This section will present the complementary features to the previous subsection~\ref{subsec:components}.
The most important feature of our framework and also the base of other features is the configuration system that we present in subsection~\ref{subsec:configs}.
Based on the configuration system, we introduce the out-of-the-box feature in subsection~\ref{subsec:outofthebox}.
In subsection~\ref{subsec:callbacks}, we will present the callback system of DIVA-DAF.
To further adapt the framework to the user's need, we will discuss the modularity of the framework in subsection~\ref{subsec:modules}.
Finally, in section~\ref{subsec:features_logging}, we will present the logging capability of our framework. 

% In this section, we will explain the different features the framework provides, their usage, and implementation.
% overview of the section

% TODO: explain the patch and whole page possibility

\subsection{Configurations}\label{subsec:configs}
% based on hydra
% created object based on the arguments in the configs
% overall config
% This makes it possible to exactly reproduce an experiment as we have all the parameters of each object stored in a file
We use configuration files to rerun an experiment quickly or share it with a colleague easily.
The configuration system of our framework is provided by Hydra~\cite{yadanHydraFrameworkElegantly2019}, which creates Python objects based on configuration files in an elegant fashion.
These configuration files contain the Python path to a class and the arguments to initialize the class.
The path can lead to a class implemented by the user or one in a Python package, e.g., Torchvision.
By combining the different configurations for the task, model, metrics, and loss, the user can create a precise definition of an experiment. 
When the framework has successfully read all configuration files, it combines them and stores this run configuration in the specific experiment output folder.
Using this experiment configuration file, we can reproduce an experiment as all the parameters of each created object are stored.

Datamodule and task objects have an additional ability. 
Configurations can use run-time variables from these objects in their definitions.
For example, the user can set the number of output filters for a segmentation network depending on the datamodule at run-time.
In Listing~\ref{lst:datamodule_example}, we show how we can use run-time information of the datamodule object in the network configuration.

% What is unique about the datamodule is that you can use values and variables in other configurations you do not know before run-time. You find an example in Listing~\ref{lst:datamodule_example} where the model needs to know the number of output classes which is identified during the setup of the datamodule.

\begin{lstlisting}[frame=single, caption={Usage of the datamodule variable \texttt{num\_classes} which is set during run-time.}, label={lst:datamodule_example}]
_target_: pl_bolts.models.vision.UNet
num_classes: ${datamodule:num_classes}
\end{lstlisting}


% - Out-of-the-box deep learning
\subsection{Out-of-the-box Deep Learning}\label{subsec:outofthebox}
% general setup
The setup of DIVA-DAF is straightforward: The user clones the code from the GitHub repository\footnote{\url{https://github.com/DIVA-DIA/DIVA-DAF}} and create a new Anaconda\cite{anaconda} environment based on the shipped environment file (\texttt{conda\_env\_gpu.yaml}).
This environment contains all dependencies with the corresponding versions to run the framework.
If a researcher wants to run the framework with GPU, TPU, HPU, MPS, or IPU support, the appropriate drivers and the correct PyTorch support packages (CUDA, ROCm, etc.) must be installed.

% default network, losses, datamodules, and tasks
In its current state, DIVA-DAF contains sample code for two different \acl{DIA} tasks: semantic segmentation and image classification.
These tasks can be combined with different datamodules (see section~\ref{subsec:components}) like DIVA-HisDB~\cite{simistiraDIVAHisDBPreciselyAnnotated2016} or CIFAR10~\cite{krizhevskyLearningMultipleLayers2009}.
Additionally, our framework provides default implementations and their corresponding configuration for models, losses, optimizers, and metrics.
For example, famous neural networks architectures like ResNet~\cite{heDeepResidualLearning2016} and U-Net~\cite{ronnebergerUnetConvolutionalNetworks2015}, or the widely used ADAM optimizer~\cite{kingmaAdamMethodStochastic2014} are part of the framework.


% % - Custom datamodules, Tasks, models, metrics, optimizer, logger, plugins, callbacks, and losses
% \subsection{Customizable}
% % it is possible not just to customize the configs but also add new functionality
% The framework's functionality is not limited to the existing classes and configurations.
% Users can manipulate the code of existing classes or introduce their own code.
% % There is not just the possibility to adapt existing classes and configurations, but you can also implement your own.
% % caused by the modular building style
% This is possible due to the modular architecture of our framework. 
% Each part of the framework is independent and can be swapped out at any time.

% % This can be done by using provided configurations and classes or by implementing new classes and introducing them to the system.
% % we provide a base class for the task as well as for the datamodule
% To implement your own task or datamodule in a convenient fashion you can inherit from the corresponding abstract base class of the desired module.
% These abstract classes provide general variables and methods, which give the user a good starting point to create their own module.
% % These classes can be inherited from or the user can implement the whole behavior by himself, if some rules are met.
% Even thought, the user if free to override methods or variables in the child class, certain methods and variables are crucial to preserve system integrity. % TODO check sentence 


\subsection{Callbacks}\label{subsec:callbacks}
The callback functionality is provided by the underlying PyTorch-Lightning~\cite{falconPyTorchLightning2019} library.
The user can inject code into specific parts of our framework with a callback.
Callbacks are self-contained programs that are invoked in a specific position in the code (see PyTorch-Lightning callback api~\footnote{\url{https://pytorch-lightning.readthedocs.io/en/latest/extensions/callbacks.html}}).
Each hook has its own set of parameters that can be used for different jobs.
For example, if the user wants to save the output of each validation batch on each device, he can create a callback and overwrite the method \texttt{on\_validation\_batch\_end()}.
This method receives the following arguments: the trainer, the task, the outputs, the batch, the batch index, and the data loader index.
Based on these arguments, the user can now store the network output of each batch.

% % Callback make it possible to add functionality without changing the current code
% Aside from implementing your own classes or manipulating the current code, the user has the possibility to inject code into the framework with callbacks. 
% explain again
% This functionality is provided by the underlying PyTorch-Lightning~\cite{falconPyTorchLightning2019} library.

We already provide callbacks to save the different parts of the model, to check the compatibility between the backbone and the header of the model, and to visualize the gradients of the different layers of the network when using the Weights and Biases logger (see Fig.~\ref{fig:wandb_gradients}).

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/WaB_gradients.PNG}
    \caption{We provide a callback to log the gradients of a neural network. Here you see the weights and biases change during training.
    % This visualizations can help finding flaws in your network or method. A step is defined as a forward pass of one batch per device.
    }
    \label{fig:wandb_gradients}
\end{figure}


% %  - Can use parts of other frameworks (e.g. torchvision models, torchmetric, bolts models, datamodules, pytorch losses and optimizers etc.)
% \subsection{Compatible} % modular (combine with compatibility)
% % modular build
% % each model can be replaced with own code or library code
% As our framework is build on top of other libraries there is a high compatibility with these libraries.
% To lower the workload for the user he can use for example an model from the well-known Torchvision~\cite{paszkePyTorchImperativeStyle2019} library and just have to create the corresponding configuration file (see listing~\ref{lst:datamodule_example}).
% % what kind of parts can we use
% The user can use library classes for the datamodule, the network models, the metrics, the losses, the optimizer, the logger, and the callbacks.
% In Table~\ref{tab:compatibility} you find a list of all libraries that are compatible with our framework and what you can use from each of them:

% \begin{table}
%     \caption{List of compatible libraries and classes at the moment of writing. The \cmark denotes that a certain library provides a certain module and \xmark~that it does not. In parentheses modules which we did not test.}\label{tab:compatibility}
%     \begin{tabular}{ P{0.17\textwidth} P{0.09\textwidth} P{0.09\textwidth} P{0.09\textwidth} P{0.12\textwidth} P{0.15\textwidth} P{0.12\textwidth} P{0.1\textwidth} }
%         \hline
%         Library &  Model & Metric & Loss & Optimizer & Datamodule & Callbacks & Logger\\
%         \hline 
%         PyTorch             & \xmark & \xmark & \cmark & \cmark & \xmark & \xmark & \xmark\\
%         Torchvision         & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark\\
%         Torchmetric         & \xmark & \cmark & \xmark & \xmark & \xmark & \xmark & \xmark\\
%         Lightning           & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark & \cmark\\
%         Bolts               & \cmark & \xmark & \xmark & \xmark & \cmark & (\cmark) & \xmark\\
%         \hline
%     \end{tabular}
% \end{table}

% If you want to change certain aspects of a class (e.g. model architecture) from a library, we recommend to copy the code and create your own implementation of the class.

%  - Can use parts of other frameworks (e.g. torchvision models, torchmetric, bolts models, datamodules, pytorch losses and optimizers etc.)
\subsection{Modules}\label{subsec:modules}
Our framework is built in a modular fashion, as described in subsection~\ref{subsec:components}.
% each model can be replaced with its own code or library code
Each module is independent and can be replaced with a third-party or user-defined implementation.
For example, we want to use U-Net~\cite{ronnebergerUnetConvolutionalNetworks2015} for a segmentation task that takes as a parameter the number of classes we want to segment.
The library Lightning-Bolts~\cite{falconFrameworkContrastiveSelfsupervised2020} contains an implementation of this architecture.
We can use this class by writing a corresponding configuration file (see listing~\ref{lst:datamodule_example}) and adding it as a model to our experiment configuration.
% As our framework is built on top of other libraries, there is a high compatibility with these libraries.
% To lower the workload for the user, he can use, for example, a model from the well-known Torchvision~\cite{paszkePyTorchImperativeStyle2019} library and have to create the corresponding configuration file (see listing~\ref{lst:datamodule_example}).
% what kind of parts can we use?
The user can use library classes for the datamodule, the network models, the metrics, the losses, the optimizer, the logger, and the callbacks.
In Table~\ref{tab:compatibility} we show a list of all libraries that are compatible with our framework and their functionality:

\begin{table*}
    \caption{List of compatible libraries and their modules at the moment of writing. The \cmark denotes that a certain library module is compatible with DIVA-DAF, \xmark~that it does not, and N/A that this library does not provide this kind of module.\\ *: Provides just Datasets and not full Datamodules}\label{tab:compatibility}
    \begin{tabular}{ p{0.14\textwidth} p{0.08\textwidth} p{0.08\textwidth} p{0.08\textwidth} p{0.11\textwidth} p{0.14\textwidth} p{0.11\textwidth} p{0.09\textwidth} }
        \hline
        Library &  Model & Metric & Loss & Optimizer & Datamodule & Callbacks & Logger\\
        \hline 
        PyTorch             & N/A & N/A & \cmark & \cmark & N/A & N/A & N/A\\
        Torchvision         & \cmark & N/A & N/A & N/A & (\cmark*) & N/A & N/A\\
        Torchmetric         & N/A & \cmark & N/A & N/A & N/A & N/A & N/A\\
        Lightning           & N/A & N/A & N/A & N/A & N/A & \cmark & \cmark\\
        Bolts               & \cmark & N/A & \cmark & N/A & \cmark & \cmark & \xmark\\
        \hline
    \end{tabular}
\end{table*}

Users of the framework also can create their own modules.
To conveniently implement a task or datamodule, the user can inherit from the corresponding abstract base class of the desired module.
These abstract classes provide general variables and methods, giving the user a good starting point for creating their modules.
% These classes can be inherited from, or the user can implement the whole behavior himself if some rules are met.
% Even though the user can override methods or variables in the child class, specific methods and variables are crucial to preserving system integrity.


% - different loggers
\subsection{Logging}\label{subsec:features_logging}
% the user has the choice of different predifined loggers (list of loggers)
To keep track of experiments, we use the logging functionality of PyTorch-Lightning.
They provide the most common loggers like Weights and Biases~\cite{biewaldExperimentTrackingWeights2020} (see Fig.~\ref{fig:wandb_example}) or Tensorboard.
The framework allows using multiple loggers simultaneously.
% a CSV logger is always running (implement that?)
Besides using a cloud-based logger, like Weights and Biases, the user can also use a local logger like the CSV logger.
The CSV logger writes all the logging information into the local experiment folder for later use.
% the user can implement or add new loggers the same way as other modules
Logging is not limited to scalar data like metric or loss information. 
It is also possible to log figures, images, or histograms, but each logger needs to do this individually.
As with all the other modules of our framework, users can also implement their own logger or adapt an existing one.
% In figure~\ref{fig:wandb_example} you can see a typical Weights and Biases dashboard.

% example image weights and biases
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.45\textwidth]{figures/WaB_example.PNG}
    \caption{A typical dashboard on Weights and Biases. On the left side we see a list of experiments and on the right side the plots of the logged information during the training stage.}
    \label{fig:wandb_example}
\end{figure}




==> sections/0X_requirements.tex <==
\section{Requirements}
% for researchers with a background in DL or a limited amount of knowledge of programming in DIA
% supervised and unsupervised experiments

% TODO say we have full requirement list (link) but here we just give a brief overview

% It should be easier for the user to execute, monitor, and create new experiments.
% An additional layer of abstraction where the network and what we are doing with the network are separated

% It should facilitate the usage of different datasets without extensive programming.
% The framework must be easy to maintain (updating of packages, changes of functionality).

% Mention that the maintenance is easy as we can update the dependencies without adaptions in the framework

% Store the run configuration and hyperparameters to easily re-execute an run

% modularity: Show that it is easy to exchange a dependency e.g. torchmetrics

% A lot of technical requirements are already covered by Pytorch lightning (hardware acceleration, logging, data distribution, callbacks, etc.)

% What requirements do we have, and what do we need additionally to be existing frameworks

==> sections/Reviews_DAS.tex <==
----------------------- REVIEW 1 ---------------------
SUBMISSION: 35
TITLE: DIVA-DAF: A Deep Learning Framework for Historical Document Image Analysis
AUTHORS: Lars Vögtlin, Paul Maergner and Rolf Ingold

----------- Summary -----------
The authors propose an experimental framework in the context of historical document image analysis. The proposed framework is based on pytorch an uses already implemented methods/models. The authors show a set of functionalities for experimental evaluation.
----------- Relevance to DAS -----------
SCORE: 1 (relevant)
----------- Significance -----------
SCORE: 0 (medium)
----------- Soundness -----------
SCORE: 0 (sound)
----------- Experimental evaluation -----------
SCORE: 0 (good, but lacking at some aspects)
----------- Clarity -----------
SCORE: 1 (easy to read and clear enough)
----------- Overall evaluation -----------
SCORE: 0 (borderline paper)
----- TEXT:
Overall the framework is interesting but it is unclear the utility for the community, in general. Research is a dynamic activities and the libraries used for experimentation evolves rapidly with time. The tools and current libraries that are now supported can become easly obsolete if not continious development is done. So the expect impact of this tool is limited.


----------------------- REVIEW 2 ---------------------
SUBMISSION: 35
TITLE: DIVA-DAF: A Deep Learning Framework for Historical Document Image Analysis
AUTHORS: Lars Vögtlin, Paul Maergner and Rolf Ingold

----------- Summary -----------
The paper presents a novel deep learning framework for historical document image analysis. A particular feature of the framework is that it is easy to use and allows rapid prototyping. Furthermore, it is compatible to a wide range of deep learning libraries.
----------- Relevance to DAS -----------
SCORE: 1 (relevant)
----------- Significance -----------
SCORE: -1 (low)
----------- Soundness -----------
SCORE: -1 (not sound)
----------- Experimental evaluation -----------
SCORE: -1 (very insufficient  or a theoretical paper)
----------- Clarity -----------
SCORE: 1 (easy to read and clear enough)
----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
The paper proposes a new deep learning framework including code examples in the paper. I am a bit surprised to see this as also other groups make their document analysis code availble. As such, I would have expected more comparisons to these works to highlight the value of the proposed paper. Also the proposed software does not seem to reach the state-of-the-art results using FCN and ResNet-18. While the idea of open source is of course great, I wonder why I should use a framework that does not reach state-of-the-art performance.


----------------------- REVIEW 3 ---------------------
SUBMISSION: 35
TITLE: DIVA-DAF: A Deep Learning Framework for Historical Document Image Analysis
AUTHORS: Lars Vögtlin, Paul Maergner and Rolf Ingold

----------- Summary -----------
The paper presents a new deep learning framework called DIVA-DAF to support research on historical document image analysis tasks and to develop techniques to reduce the need for manually-labeled ground truth. The framework is presented to permit the use of different kinds of training data, to perform rapid prototypes
and reproducible experiments. They propose to apply it on a semantic segmentation tasks on historical documents.
----------- Relevance to DAS -----------
SCORE: 1 (relevant)
----------- Significance -----------
SCORE: -1 (low)
----------- Soundness -----------
SCORE: -1 (not sound)
----------- Experimental evaluation -----------
SCORE: 0 (good, but lacking at some aspects)
----------- Clarity -----------
SCORE: 0 (readable, but hard to follow several points.)
----------- Overall evaluation -----------
SCORE: -1 (weak reject)
----- TEXT:
The objective is very valuable for the community.
The intro is a bit imprecise about the objectives of image analysis of ancient documents: it would have been interesting to specify the objectives  : layout segmentation, line detection, information extraction, recognition...

This type of tools seems to be designed for deep learning users (and not necessarily for designers of more recent or renovated architectures): this could have been announced in the introduction. 

Some questions can be raised:

- the state of the art is interesting in terms of references, but how does the proposal differ from others, as we find the concepts of reproducibility, rapid prototyping, and deep technologies also present in the literature

- The principle of reproducible research is very valuable and increasingly in demand. The notion of reproducibility that is announced in the introduction could be presented in relation to variety of application datasets that can not be designed in a single format. In that sens, we also wonder why the framework is specific to historical documents

- What are the justifications that allow us to assert that we can keep the same training environments (and weight of networks) on applications involving old documents of different origins or different periods?


Clarifications:

* section 3: specifies the notion of "task" => "the framework supports training on different tasks

* on figure 2 the functional boxes (which are processes, workflows or deep architectures) "model" "task" or "trainer" should be represented with another graphical convention than the calculation modules "loss", "metric" or "optimizer" or the small components "callback" or "plugin

* in the structure of the paper the section related to the definition of the plugin part does not appear and its role remains unclear

* the paper states that the framework is intended to limit the manual labeling of documents (for ground-truth): this part does not seem to be presented or evaluated

Finally in the paper, we also wonder about the possibility to update such an architecture with recent versions of deep networks. Is there any possibility of incremental update?

==> sections/old_example.tex <==
\section{Application}



A typical task in historical \acf{DIA} is semantic segmentation.
Each pixel of an input image gets assigned one of a predefined set of classes.
This output can further be used for tasks like text line segmentation~\cite{albertiLabelingCuttingGrouping2019} or handwriting recognition~\cite{joHandwrittenTextSegmentation2019}.

% U-Net Semantic segmentation DIVAHisDB
We present how to perform semantic segmentation on the Cod. Bodmer 55 of the well known DIVA-HisDB~\cite{simistiraDIVAHisDBPreciselyAnnotated2016} dataset (see Fig.~\ref{fig:dataset}). 
The dataset contains 20 pages for training, 10 pages for validation, and 10 pages for testing. Each page has a dimension of 4872$\times$6496 pixels with a resolution of 600 dpi.
Each pixel belongs to one of 8 classes (background, main text body, decoration, comment, main text body + comment, main text body + decoration, comment + decoration,  main text body + decoration + comment).

% Example Image CB55
\begin{figure*}[ht] 
    \centering
    
    \subfloat[CB55, p. 25r]{
    \includegraphics[width=\columnwidth]{figures/example_data/cb55_0025r_cropped.jpg}\label{fig:dataset_cb55_A}}
    \hfill
    \subfloat[CB55, p. 5v]{
    \includegraphics[width=\columnwidth]{figures/example_data/cb55_5v_cropped.jpg}\label{fig:dataset_cb55_B}}
    
    \caption{
    Sample pages of the medieval manuscripts Cod. Bodmer 55 of DIVA-HisDB.
    }
    \label{fig:dataset}
\end{figure*}

% explain setup
DIVA-DAF provides a task module for semantic segmentation. We have to select a datamodule and bring the dataset into the expected format.
We decide to process the page in crops of size 256$\times$256 pixel because of the size of the full-page images. Precisely, we have prepared the training and validation data by cropping each page into 1376 300$\times$300 pixel patches with 50\% overlap. Then, we take a random 256$\times$256 crop from each patch during each training and validation epoch. Accordingly, we select the datamodule available in DIVA-DAF that works with this kind of data (\texttt{DIVAHisDB/datamodule\_cropped.py}). 

We use a random initialized vanilla U-Net~\cite{ronnebergerUnetConvolutionalNetworks2015} architecture ($\sim$31 million parameters), which has eight output layers.
The network was trained using the ADAM~\cite{kingmaAdamMethodStochastic2014} optimizer with a learning rate of \texttt{0.001} for \texttt{50} epochs with a batch size of 16.
As a loss, we used the Cross-Entropy loss.
We run all of our experiments on a server with 4 $\times$ NVIDIA 1080 GTX with 8GB of GPU memory each, an Intel i7-5960X CPU, and 64 GB of RAM.
To evaluate the networks output after testing we use the official evaluation tool~\cite{albertiOpenEvaluationTool2017a} of the ICDAR 2017 competition~\cite{simistiraICDAR2017CompetitionLayout2017}.
The tool computes the \ac{mIoU} and the F1-score between the prediction of our network and the ground truth.

% explain and write down the run command and the configuration
In our repository you will find under \texttt{configs/experiment} a file \texttt{cb55\_full\_run\_unet.yaml}, that contains all above listed parameters and configurations.
We will train the network with the train/val split and automatically execute the testing routine after training.
To run this experiment you start the framework with the following command:
\begin{lstlisting}
$ python run.py experiment=cb55_full_run_unet.yaml
\end{lstlisting}

% how would that look, and what are the results
The run logs and the output of the testing stage will be stored in the experiment directory.
Each setup (30, 15, 1 training page(s)) was executed three times with three different seeds and then averaged.
We used for the three different setups always the same three seeds for the runs.
Using the same seeds ensures that the experiments start with the same initial network weights.
% TODO is this really needed?
% To run the experiment with 15 training pages and the seed 2149823 the command would look like the following:
% \begin{lstlisting}
% $ python run.py experiment=cb55_full_run_unet.yaml 
%     datamodule.selection_train=15 +seed=2149823
% \end{lstlisting}

A configuration file change is not needed to run the experiment if only a few parameters need to be changed. Instead, parameters can be changed or added as a command-line argument. 
In this experiment, we only want to adjust the number of training pages and seeds, which we can do more quickly using the command line. 
The following command shows how to run the base experiment with 15 training pages and a seed of 2149823.
\begin{lstlisting}
$ python run.py experiment=cb55_full_run_unet.yaml 
    datamodule.selection_train=15 +seed=2149823
\end{lstlisting}

%% result table (full, 15, 1)
% competition results - top 2
% TODO check table columns
\begin{table*}[h]
    \caption{Results of semantic segmentation on the testset of DIVA-HisDBs CB55 with a U-Net. All results are averages over three runs with different random seeds. All our networks were trained for 50 epochs.}
    \label{tab:segmentation_results}
    \begin{tabular}{ p{0.07\textwidth} p{0.07\textwidth} p{0.14\textwidth} p{0.15\textwidth} p{0.13\textwidth} p{0.14\textwidth} p{0.14\textwidth}}
        \hline
        Authors & Year & \#train pages & Model & Run time & \ac{mIoU}[\%] & F1-Score[\%] \\
        \hline
        % Studer et al.~\cite{studerComprehensiveStudyImageNet2019a} & 30 & SegNet  & $\sim$8h    & 86.90 & N/A\\
        % Studer et al.~\cite{studerComprehensiveStudyImageNet2019a} & 30 & DeepLabV3     & $\sim$8h    & 92.90 & N/A\\
        % System-5~\cite{simistiraICDAR2017CompetitionLayout2017} & 30 & FCN$^\ast$ & N/A   & 98.35 & N/A\\
        % System-4.1~\cite{simistiraICDAR2017CompetitionLayout2017}& 30 & ResNet18     & N/A    & 98.64 & N/A\\
        \cite{studerComprehensiveStudyImageNet2019a} & 2019 & 20 & SegNet  & $\sim$8h    & 86.90 & N/A\\
        \cite{studerComprehensiveStudyImageNet2019a} & 2019 & 20 & DeepLabV3  & $\sim$8h & 92.90 & N/A\\
        \cite{simistiraICDAR2017CompetitionLayout2017} & 2017 & 20 & FCN$^\ast$ & N/A   & 98.35 & N/A\\
        \cite{simistiraICDAR2017CompetitionLayout2017} & 2017 & 20 & ResNet18     & N/A    & 98.64 & N/A\\
        \hline
        Ours & 2022 & 1  & U-Net & $\sim$0.25h & 90.93$\pm$3.09 & 94.93$\pm$1.89\\
        Ours & 2022 & 15 & U-Net & $\sim$2.75h & 96.33$\pm$0.44 & 98.03$\pm$0.20\\
        Ours & 2022 & 20 & U-Net & $\sim$3.5h  & 97.26$\pm$0.20 & 98.63$\pm$0.11\\
        \hline
    \end{tabular}
    $^\ast$: Fully-convolutional Neural Network
\end{table*}
% SegNet~\cite{badrinarayananSegNetDeepConvolutional2017}
% DeepLabV3~\cite{chenRethinkingAtrousConvolution2017}
% ResNet18~\cite{heDeepResidualLearning2016}

% evtl remove 15 column
\begin{table}
    \centering
    \caption{Visual results of semantic segmentation on the testset of DIVA-HisDBs CB55 with a U-Net. In the images you see comments(red), main text(purple), decoration(yellow), and main text + decoration(turquoise). We can see that the quality of the segmentation decreases with the amount of training pages.}
    \label{tab:segmentation_results_images}
    \begin{tabular}{ p{0.18\textwidth} | p{0.39\textwidth} p{0.39\textwidth} }
        & &\\
        &  CB55 p. 98v & CB55 p. 102v \\
        \hline
        
        & &\\
        
        \parbox[m]{0.17\textwidth}{ \vspace*{-7em} Original} &
        \includegraphics[scale=.78]{figures/result_images/cb55-98v/e-codices_fmb-cb-0055_0098v_max-series-ori.pdf} & \includegraphics[scale=.8]{figures/result_images/cb55-102v/e-codices_fmb-cb-0055_0102v_max-series-ori.pdf} \\
        
        & &\\
        \parbox[m]{0.17\textwidth}{ \vspace*{-7em} 30 Pages} &
        \includegraphics[scale=.78]{figures/result_images/cb55-98v/e-codices_fmb-cb-0055_0098v_max-series-30.pdf} &
        \includegraphics[scale=.8]{figures/result_images/cb55-102v/e-codices_fmb-cb-0055_0102v_max-series-30.pdf} \\
       
        & &\\
        \parbox[m]{0.17\textwidth}{ \vspace*{-7em}15 Pages} &
        \includegraphics[scale=.78]{figures/result_images/cb55-98v/e-codices_fmb-cb-0055_0098v_max-series-15.pdf} &
        \includegraphics[scale=.8]{figures/result_images/cb55-102v/e-codices_fmb-cb-0055_0102v_max-series-15.pdf}\\
       
        & &\\
        \parbox[m]{0.17\textwidth}{ \vspace*{-7em}1 Page} &
        \includegraphics[scale=.78]{figures/result_images/cb55-98v/e-codices_fmb-cb-0055_0098v_max-series-1.pdf} &
        \includegraphics[scale=.8]{figures/result_images/cb55-102v/e-codices_fmb-cb-0055_0102v_max-series-1.pdf}\\
      
        & &\\
        \parbox[m]{0.17\textwidth}{ \vspace*{-7em}Ground Truth} &
        \includegraphics[scale=.78]{figures/result_images/cb55-98v/e-codices_fmb-cb-0055_0098v_max-series-gt.pdf} &
        \includegraphics[scale=.8]{figures/result_images/cb55-102v/e-codices_fmb-cb-0055_0102v_max-series-gt.pdf}\\
        
        \hline
    \end{tabular}
\end{table}

% we have good results
% sota compared to the other results
In Table~\ref{tab:segmentation_results} the averages of the different setups we ran and some state-of-the-art results.
We can see that our system with 30 training pages is close to the current state-of-the-art reported in the ICDAR 2017 competition~\cite{simistiraICDAR2017CompetitionLayout2017}.
With 15 pages our model outperforms both the SegNet and the DeepLabV3 reporeted by Studer et al.~\cite{studerComprehensiveStudyImageNet2019a}.
Even with one training page, we outperform the SegNet, and we achieve this with a training time of $\sim$0.25h.
An explanation could be that the first page of the training set is an excellent overall representation of the dataset.

In Table~\ref{tab:segmentation_results_images}, you can observe that the segmentation quality decreases with fewer training examples.
Additionally, we can see that all setups struggle in certain sections to separate main text and comments.
Overall, every setup produces precise contours and has a clean border between classes.

% -----------------------------

% We already did multiple publications with this framework as well as experiments for a phd thesis

% feedback Vinay: it took me all of 10 minutes to run something first, and 1h to make my own modifications. Very nice and modular!

% we will add the experiment from the old paper but we will point out, that we are measuring the time and not the performance.



Base step: Implementing the different parts (dataset + datamodule including statistics and cutting the images)

\#1: load just the first 3 layers of the encoder of the unet
\#2: change the network with the same task
\#3: adapt the task for both networks
\begin{table*}
  \caption{Implementation Time in minutes and code douplication in lines of code}
  \label{tab:commands}
  \begin{tabular}{lcccc}
    \toprule
    Module part & \multicolumn{2}{c}{Implementation time [m]} & \multicolumn{2}{c}{Code Duplication}\\
                & Scratch & DIVA-DAF & Scratch & DIVA-DAF\\
    \midrule
    Data loading            & 150 & 10 & 0 & 0 \\
    Network                 & 30  & 5  & 0 & 0 \\
    Execution               & 10  & 10 & 0 & 0 \\
    \midrule
    Load a Network Part     & 15 & 2 & 0 & 0 \\
    New network; same task  &  &  &  &  \\
    Adapt the task          &  &  &  &  \\
    \bottomrule
  \end{tabular}
\end{table*}

